Word Rotator's Distance

A key principle in assessing textual similarity is measuring the degree of semantic overlap between two texts by considering the word alignment. Such alignment-based approaches are intuitive and interpretable; however, they are empirically inferior to the simple cosine similarity between general-purpose sentence vectors. To address this issue, we focus on and demonstrate the fact that the norm of word vectors is a good proxy for word importance, and their angle is a good proxy for word similarity. Alignment-based approaches do not distinguish them, whereas sentence-vector approaches automatically use the norm as the word importance. Accordingly, we propose a method that first decouples word vectors into their norm and direction, and then computes alignment-based similarity using earth mover's distance (i.e., optimal transport cost), which we refer to as word rotator's distance. Besides, we find how to grow the norm and direction of word vectors (vector converter), which is a new systematic approach derived from sentence-vector estimation methods. On several textual similarity datasets, the combination of these simple proposed methods outperformed not only alignment-based approaches but also strong baselines. The source code is available at https://github.com/eumesy/wrd

==> alg/alg_WMD.tex <==
\begin{algorithmic}[1]
\Input{a pair of sentences $S=\{\mathbf w_1,\dots,\mathbf w_n\}$, $S'=\{\mathbf w'_1,\dots,\mathbf w'_m\}$}
\State{Compute histograms:}
\Let{\mathbf h_S}{(1/n,\dots,1/n) \in \mathbb R^n}
\Let{\mathbf h_{S'}}{(1/m,\dots,1/m) \in \mathbb R^m}
\State{Compute cost matrix $\mathbf C \in \mathbb R^{n \times m}$:}
\For{$i \gets 1$ to $n$}
\For{$j \gets 1$ to $m$}
\Let{\mathbf C_{ij}}{\lVert \mathbf w_i - \mathbf w'_j\rVert_2}
\EndFor
\EndFor
\State{Compute earth mover's distance:}
\Let{d(S,S')}{\textsc{EMD}(\mathbf h_S, \mathbf h_{S'}; \mathbf C)}
\Output{
dissimilarity $d(S,S')$
}
\end{algorithmic}

